The Cosmological Parameters (2019)

This is a review article for The Review of Particle Physics 2020 (aka the Particle Data Book). It forms a compact review of knowledge of the cosmological parameters at the end of 2019. Topics included are Parametrizing the Universe; Extensions to the standard model; Probes; Bringing observations together; Outlook for the future.

==> hubble-allref.tex <==
%!TEX root = hubble.tex
% AL (16 Sep 2019)
 
\referencelist 
 
\reference{hubble:planck2018I} Planck Collab.\ 2018 Results I, arXiv:1807.06205\rm   
\endreference
 
\reference{hubble:planck2018VI} Planck Collab.\ 2018 Results VI,
arXiv:1807.06209v2\rm
\endreference
 
\reference{hubble:wmap9be} C. Bennett \etal, \ajs208,20(2013)\rm
\endreference 
 
\reference{hubble:wmap9hi} G. Hinshaw \etal, \ajs208,19(2013)\rm
\endreference 
 
\reference{hubble:solosc} S. Fukuda \etal, \prl85,3999(2000)  
\endreference 
 
\reference{*hubble:xxx} Q.R. Ahmad \etal, \prl87,071301(2001) 
\endreference 
 
\reference{hubble:inf} E.W. Kolb and M.S. Turner, {\it The Early
Universe}\rm, Addison--Wesley (Redwood City, 1990)  
\endreference 
 
\reference{hubble:PDP} D.H. Lyth and A.R. Liddle, {\it The Primordial Density 
Perturbation}\rm, Cambridge University Press (2009) 
\endreference 

\reference{hubble:LL}
A.R. Liddle and D.H. Lyth, \plB291,391(1992)
\endreference
 
\reference{hubble:Boltz} A. Lewis, A Challinor, and
A. Lasenby, \aj538,473(2000)     
\endreference 
 
\reference{*hubble:xxx}  D. Blas, J. Lesgourgues, and
T. Tram, \jcap1107,034(2011)     
\endreference 
  
\reference{hubble:fix} D. Fixsen, \aj707,916(2009) 
\endreference 

\reference{hubble:hobson} M. Hobson \etal (eds). {\it Bayesian
Methods in Cosmology}, Cambridge University Press (2009)  
\endreference 
 
\reference{hubble:KT} A. Kosowsky and M.S. Turner, \prD52,1739(1995) 
\endreference 
 
\reference{hubble:mw} K.A. Malik and D. Wands, \prept475,1(2009) 
\endreference 
 
\reference{hubble:planckXXV} Planck Collab.\ 2013 Results
XXV, \aap571,A25(2014)\rm 
\endreference 
 
\reference{hubble:curv} D.H. Lyth and D. Wands, \plB524,5(2002)  
\endreference 
 
\reference{*hubble:xxx} K. Enqvist and M.S. Sloth, \npB626,395(2002)
\endreference 
 
\reference{*hubble:xxx} T. Moroi and T. Takahashi, \plB522,215(2001)
\endreference 
 
\reference{hubble:sp16}  P. F. de Salas and S. Pastor, \jcap1607,051(2016)
\endreference
 
\reference{hubble:Neff}  S. Riemer-S{\o}rensen, D. Parkinson, and
T.M. Davis, Pub. Astron. Soc. Pacific {\bf 30}, e029 (2013)  
\endreference
 
\reference{hubble:Webb} J.K. Webb \etal, \prl107,191101(2011)
\endreference 
 
\reference{*hubble:xxx} J.A. King \etal, \mnras422,3370(2012) 
\endreference 
 
\reference{*hubble:xxx} P. Molaro \etal, \aap555,68(2013)  
\endreference 

\reference{hubble:planck2015XVIII} Planck Collab.\ 2015 Results 
XVIII, \aap594,A18(2016)\rm  
\endreference 
  
\reference{hubble:freedman} W.L. Freedman \etal, \aj553,47(2001) 
\endreference 
 
%\reference{hubble:riess16} A.G. Riess  \etal, Astrophys. J. {\bf 826},
%56 (2016)   
%\endreference 

\reference{hubble:riess19} A.G. Riess  \etal, \aj876,85(2019)
\endreference 

\reference{hubble:freedman2019} W.L. Freedman \etal, \aj882,34(2019)
\endreference 

\reference{hubble:Holicow}  K.C. Wong \etal, arXiv:1907.04869 (2019)
\endreference 

\reference{hubble:bright_siren} B.P. Abbott \etal, \nature551,85(2017) 
\endreference 

\reference{hubble:dark_siren} M. Soares-Santos \etal, \ajl876,L7(2019)
\endreference 

\reference{hubble:inverse_ladder} E. Macaulay  \etal, \mnras486,2184(2019)
\endreference 

 \reference{hubble:DESY1_BAO_BBN} T.M.C. Abbott \etal,  \mnras480,3879(2018)
 \endreference 

\reference{verde} L. Verde. T. Treu, and A. G. Riess, arXiv:1907.10625 (2019)
\endreference

%\reference{hubble:humphreys13} E.M.L. Humphreys \etal,
%Astrophys. J.,775, 13 (2013) 
%\endreference

\reference{hubble:leibundgut} B. Leibundgut, \araa39,67(2001)  
\endreference 
 
\reference{hubble:snfirst} A.G. Riess \etal, Astron.\ J.\ {\bf 116},
1009 (1998)  
\endreference 
 
\reference{*hubble:xxx} P. Garnavich \etal, \aj509,74(1998) 
\endreference 
 
\reference{*hubble:xxx} S. Perlmutter \etal, \aj517,565(1999)
\endreference 
 
%\reference{hubble:SNLS3} A. Conley \etal, \ajs192,1(2011)   
%\endreference 
 
%\reference{*hubble:xxx} M. Sullivan \etal, \aj737,102(2011) 
%\endreference 
 
%\reference{hubble:kowalski} M. Kowalski  \etal, \aj686,749(2008) 
%\endreference 
 
%\reference{hubble:kessler} R. Kessler  \etal, \ajs185,32(2009) 
%\endreference 

\reference{hubble:betoule14} M. Betoule \etal,  \aap568,22(2014)
\endreference

\reference{hubble:DES_SNeIa} T.M.C. Abbott \etal,  \ajl872,2(2018)
\endreference 

%\reference{hubble:DES} Abbott  \etal,  Astron. \&
%Astrophys., 568, 22 (2014)
%\endreference
 
\reference{hubble:LewBrid} A. Lewis and S. Bridle, \prD66,103511(2002) 
\endreference 
 
\reference{hubble:cosmosis} J. Zuntz \etal, Astronomy and Computing {\bf 12}, 45 (2015)
\endreference

\reference{hubble:cosmolike} E. Krause and T. Eifler, \mnras470,2100(2017)
\endreference

%\reference{hubble:DASI} J. Kovac \etal, \nature420,772(2002)
%\endreference 
 
%\reference{hubble:Das} S. Das \etal, \prl107,021301(2011) 
%\endreference 

\reference{hubble:Kaiser84} N. Kaiser, \aj284,L9(1984) 
\endreference 

\reference{hubble:DL99} A. Dekel and O. Lahav,  \aj520,24(1999) 
\endreference 
 
\reference{hubble:eisenstein05} D. Eisenstein  \etal, \aj633,560(2005) 
\endreference 
 
\reference{hubble:cole05} S. Cole  \etal, \mnras362,505(2005) 
\endreference 
 
%\reference{hubble:boss13} A. Sanchez \etal, \mnras433,1202(2013)\rm
%\endreference 
 
%\reference{hubble:boss14} L. Anderson \etal, \mnras441,24(2014)\rm
%\endreference 
 
 \reference{hubble:boss17} S. Alam \etal, \mnras470, 2617(2017)\rm
\endreference 

 \reference{hubble:parkinson13} D. Parkinson \etal, \prD86,103518(2012)\rm
\endreference 
 
%\reference{hubble:blake11} C. Blake  \etal, \mnras418,1707(2011) 
%\endreference 
 
\reference{hubble:kaiser} N. Kaiser, \mnras227,1(1987) 
\endreference 
 
\reference{hubble:guzzo} L.  Guzzo \etal, \nature451,541(2008) 
\endreference 
 
\reference{hubble:nusser11} A. Nusser and M. Davis, \aj736,93(2011) 
\endreference 

\reference{hubble:ap1979}  C. Alcock and B. Paczynski, \nature281, 358 (1979)
\endreference 

\reference{hubble:blake12} C. Blake \etal, \mnras425,405(2012)\rm
\endreference

\reference{hubble:BOSS16}
H. Gil-Mar\'{\i}n \etal, \mnras465,1757(2017)
\endreference

\reference{hubble:lp06} J. Lesgourgues and  S. Pastor, \prept429,307(2006) 
\endreference 
 
%\reference{hubble:thomas10} S. Thomas, F.B. Abdalla, and O. Lahav, 
%\prl105,031301(2010)  
%\endreference 
  
%\reference{hubble:boss_nu12} G.-B. Zhao  \etal, \mnras436,2038(2013)\rm 
%\endreference

%\reference{hubble:wigglez_nu12}
%S. Riemer-S{\o}rensen \etal, \prD85,081101(2012)  
%\endreference

%\reference{hubble:slosar13}
%A. Slosar \etal, JCAP {\bf 1404}, 026 (2014)\rm
%\endreference

%\reference{hubble:delubac} T. Delubac \etal, Astron. \&
%Astrophys. {\bf 574}, A59 (2015)
%\endreference

\reference{hubble:lya1}
M. Blomqvist  \etal, \aap629,A86(2019)
\endreference

\reference{hubble:lya2}
A. de Sainte \etal, \aap629,A85(2019)
\endreference

\reference{hubble:viel13}
M. Viel \etal, \prD88,043502(2013)\rm
\endreference

\reference{hubble:lensing}  A. Refregier, \araa41,645(2003) 
\endreference 
 
\reference{*hubble:xxx} R. Massey \etal, \nature445,286(2007) 
\endreference 
 
\reference{*hubble:xxx} H. Hoekstra and B. Jain, \arnps58,99(2008) 
\endreference 
 
\reference{hubble:KiDS18}  H. Hildebrandt \etal, arXiv:1812.06076 (2018)
\endreference 

\reference{hubble:Troxel18}  M. Troxel \etal, \prD98,043528(2018)
\endreference 

 \reference{hubble:Higake18}  M. Higake \etal, Pub. Astron. Soc. Japan {\bf 71}, 43 (2018)
\endreference 

\reference{hubble:isw1} R.G. Crittenden and N. Turok, \prl75,2642(1995) 
\endreference 
 
%\reference{hubble:tg13} T. Giannatonio \etal, \mnras426,258(2012)
%\endreference

%\reference{hubble:planck2015XI} Planck Collab.\ 2015 Results XI,
%Astron. \& Astrophys. {\bf 594}, A11 (2016)\rm 
%\endreference 

\reference{hubble:planckXXI} Planck Collab.\ 2015 Results
XIX, \aap594,A21(2016)\rm  
\endreference

\reference{hubble:planckXXIV} Planck Collab.\ 2015 Results
XX, \aap594,A24(2016)\rm  
\endreference 
   
%\reference{hubble:cfhtlens13} M. Kilbinger \etal, \mnras430,2200(2013)
%\endreference
 
%\reference{*hubble:xxx} C. Heymans \etal, \mnras427,146(2012)
%\endreference

%\reference{*hubble:xxx} C. Heymans \etal, \mnras432,2433(2013)
%\endreference

%\reference{hubble:deswl15} Dark Energy Survey Collab.,
%\prD94,022001(2016)\rm
%\endreference

\reference{hubble:dekel} A. Dekel, \araa32,371(1994) 
\endreference 
 
%\reference{hubble:planck2015XX} Planck Collab.\ 2015 Results XX,
%Astron. \& Astrophys. {\bf 594}, A20 (2016)\rm 
%\endreference 

\reference{alam17}
S. Alam \etal, \mnras470,2617(2017)\rm
\endreference

\reference{hubble:planck2018X} Planck Collab.\ 2018 Results X,
arXiv:1807.06211v2\rm
\endreference

\reference{hubble:planck2018IX} Planck Collab.\ 2018 Results IX,
arXiv:1905.05697\rm 
\endreference 

\reference{hubble:KiDS}  E. van Uitert \etal,  \mnras476,4662(2018)\rm 
\endreference

\reference{hubble:DESY1}  DES Collab., \prD98,043526(2018)\rm 
\endreference 


\endreferencelist 


==> hubble-body.tex <==
%!TEX root = hubble.tex
\BleederPointer=7
%% \font\tencaps=cmcsc10

%-----------------------------

% 2019 version, proposed initial submission version 4-Aug-2019 by AL
% 2019 version, revised  2-Aug-2019 by OL
% 2019 version, minor corrections 29-July-2019 by AL
% 2019 version, revised  29-July-2019 by OL
% 2019 version, initiated 12-July-2019 by AL
%
%---------------------------
\IndexEntry{hubblepage}
\heading{Cosmological Parameters}
%Redefine upper case greek letters so that particle names are slanted
%Make new definitions to correspond to old definitions
\mathchardef\OMEGA="700A

\beginRPPonly
\runninghead{Cosmological parameters}
\IndexEntry{hubbleCosmParam}

\def\paragraph#1{\medskip\noindent\bgroup\boldface\bfit #1:\egroup}
\def\mnras#1,#2(#3){{\rm MNRAS\ }{\bf #1}, {\rm#2} {\rm(#3)}}

\overfullrule=5pt

\ifnum\WhichSection=7
\magnification=\magstep1
\fi

%Redefine upper case greek letters so that particle names are slanted
%Make new definitions to correspond to old definitions
\mathchardef\OMEGA="700A
\mathchardef\OMEGA="700A
\WhoDidIt{Updated September 2019, by O.\ Lahav (University College London) % 
and A.R.\ Liddle (Perimeter Institute for Theoretical Physics and Universidade de Lisboa).}%\WhoDidIt

%% \def\kmsMpc{km~s$^{-1}$~Mpc$^{-1}$}

\ifnum\WhichSection=7
\else
\advance\baselineskip by -.2pt
\fi

\def\ltsima{$\; \buildrel < \over \sim \;$}
\def\simlt{\lower.5ex\hbox{\ltsima}} \def\gtsima{$\; \buildrel > \over
\sim \;$} \def\simgt{\lower.5ex\hbox{\gtsima}}


\section{Parametrizing the Universe}


%\begin{figure}[h]
%\includegraphics[width=8cm]{H0_Verde.pdf}
%\end{figure}


Rapid advances in observational cosmology have led to the
establishment of a precision cosmological model, with many of the key
cosmological parameters determined to one or two significant figure
accuracy. Particularly prominent are measurements of cosmic microwave
background (CMB) anisotropies, with the highest precision observations
being those of the {\it Planck}
Satellite\cite{hubble:planck2018I}\cite{hubble:planck2018VI} which
supersede the landmark {\it WMAP}
results\cite{hubble:wmap9be}\cite{hubble:wmap9hi}. However the most
accurate model of the Universe requires consideration of a range of
observations, with complementary probes providing consistency checks,
lifting parameter degeneracies, and enabling the strongest constraints
to be placed.

The term `cosmological parameters' is forever increasing in its scope,
and nowadays often includes the parameterization of some functions, as
well as simple numbers describing properties of the Universe. The
original usage referred to the parameters describing the global
dynamics of the Universe, such as its expansion rate and
curvature. Now we wish to know how the matter budget of the
Universe is built up from its constituents: baryons, photons,
neutrinos, dark matter, and dark energy. We also need to describe the
nature of perturbations in the Universe, through global statistical
descriptors such as the matter and radiation power spectra. There may
be additional parameters describing the physical state of the Universe, such
as the ionization fraction as a function of time during the era since
recombination.  Typical comparisons of cosmological models with
observational data now feature between five and ten parameters.

\subsection{The global description of the Universe}

Ordinarily, the Universe is taken to be a perturbed Robertson--Walker
space-time, with dynamics governed by Einstein's equations. This is
described in detail in the Big-Bang Cosmology chapter in this volume.
Using the density parameters $\OMEGA_i$ for the various matter species
and $\OMEGA_\LAMBDA$ for the cosmological constant, the Friedmann
equation can be written
$$
\sum_i \OMEGA_i + \OMEGA_\LAMBDA -1 = \frac{k}{R^2 H^2} \,,
\EQN{redfried}
$$
where the sum is over all the different species of material in the
Universe. This equation applies at any epoch, but later in this
article we will use the symbols $\OMEGA_i$ and $\OMEGA_\LAMBDA$ to
refer specifically to the present-epoch values.

The complete present-epoch state of the homogeneous Universe can be
described by giving the current-epoch values of all the density
parameters and the Hubble constant $h$ (the present-day Hubble
parameter being written $H_0 = 100 h \, {\rm km}\,{\rm s}^{-1}\,{\rm
Mpc}^{-1}$).  A typical collection would be baryons $\OMEGA_{{\rm
b}}$, photons $\OMEGA_\gamma$, neutrinos $\OMEGA_\nu$, and cold dark
matter $\OMEGA_{{\rm c}}$ (given charge neutrality,
the electron density is guaranteed to be too small to be worth
considering separately and is effectively included with the baryons).
The spatial curvature can then be determined from the other parameters
using \Eq{redfried}. The total present matter density $\OMEGA_{{\rm
m}} =\OMEGA_{{\rm c}}+\OMEGA_{{\rm b}}$ may be used in place of
the cold dark matter density $\OMEGA_{{\rm c}}$.

\newpage % New page forced by hand as otherwise page 1 is over length
         % for some reason.

These parameters also allow us to track the history of the Universe,
at least back until an epoch where interactions allow interchanges
between the densities of the different species; this is believed to
have last happened at neutrino decoupling, shortly before Big-Bang
Nucleosynthesis (BBN).  To probe further back into the Universe's
history requires assumptions about particle interactions, and perhaps
about the nature of physical laws themselves.

The standard neutrino sector has three flavors. For neutrinos of mass
in the range $5 \times 10^{-4} \, {\rm eV}$ to $1\,{\rm MeV}$, the
density parameter in neutrinos is predicted to be
$$
\OMEGA_\nu h^2 = \frac{\sum m_\nu}{93.14 \, {\rm eV}} \,,
\EQN{}
$$
where the sum is over all families with mass in that range (higher
masses need a more sophisticated calculation). We use units with $c=1$
throughout. Results on atmospheric and Solar neutrino
oscillations\cite{hubble:solosc} imply non-zero mass-squared
differences between the three neutrino flavors.  These oscillation
experiments cannot tell us the absolute neutrino masses, but within
the simple assumption of a mass hierarchy suggest a lower limit of
approximately $0.06 \, {\rm eV}$\IndexEntry{hubbleNuDens} for the sum
of the neutrino masses (see the Neutrino chapter).

Even a mass this small has a potentially observable effect on the
formation of structure, as neutrino free-streaming damps the growth of
perturbations. Analyses commonly now either assume a neutrino mass sum
fixed at this lower limit, or allow the neutrino mass sum to be a
variable parameter. To date there is no decisive evidence of any
effects from either neutrino masses or an otherwise non-standard
neutrino sector, and observations impose quite stringent limits; see
the Neutrinos in Cosmology chapter.  However, we note that the
inclusion of the neutrino mass sum as a free parameter can affect the
derived values of other cosmological parameters.

\subsection{Inflation and perturbations}
\IndexEntry{hubbleInflation}

A complete model of the Universe should include a description of
deviations from homogeneity, at least in a statistical way. Indeed,
some of the most powerful probes of the parameters described above
come from the evolution of perturbations, so their study is naturally
intertwined with the determination of cosmological parameters.

There are many different notations used to describe the perturbations,
both in terms of the quantity used to and
the definition of the statistical measure. We use the dimensionless
power spectrum $\Delta^2$ as defined in the Big Bang Cosmology section
(also denoted ${\cal P}$ in some of the literature). If the
perturbations obey Gaussian statistics, the power spectrum provides a
complete description of their properties.

From a theoretical perspective, a useful quantity to describe the
perturbations is the curvature perturbation ${\cal R}$, which measures
the spatial curvature of a comoving slicing of the space-time.  A
simple case is the
\IndexEntry{hubbleHZeldovich}Harrison--Zeldovich spectrum, which
corresponds to a constant $\Delta^2_{{\cal R}}$. More generally, one
can approximate the spectrum by a power law, writing
$$
\Delta^2_{{\cal R}}(k) = \Delta^2_{{\cal R}}(k_*) 
\left[\frac{k}{k_*}\right]^{n_{{\rm s}}-1} \,,
\EQN{}
$$
where $n_{{\rm s}}$ is known as the spectral index, always defined so
that $n_{{\rm s}}=1$ for the Harrison--Zeldovich spectrum, and $k_*$
is an arbitrarily chosen scale.  The initial spectrum, defined at some
early epoch of the Universe's history, is usually taken to have a
simple form such as this power law, and we will see that observations
require $n_{{\rm s}}$ close to one. Subsequent evolution will modify
the spectrum from its initial form.

The simplest mechanism for generating the observed perturbations is
the inflationary cosmology, which posits a period of accelerated
expansion in the Universe's early
stages\cite{hubble:inf}\cite{hubble:PDP}. It is a useful working
hypothesis that this is the sole mechanism for generating
perturbations, and it may further be assumed to be the simplest class
of inflationary model, where the dynamics are equivalent to that of a
single scalar field $\phi$ with canonical kinetic energy slowly
rolling on a potential $V(\phi)$. One may seek to verify that this
simple picture can match observations and to determine the properties
of $V(\phi)$ from the observational data. Alternatively, more
complicated models, perhaps motivated by contemporary fundamental
physics ideas, may be tested on a model-by-model basis (see more in
the Inflation chapter in this volume).

Inflation generates perturbations through the amplification of quantum
fluctuations, which are stretched to astrophysical scales by the rapid
expansion. The simplest models generate two types, density
perturbations that come from fluctuations in the scalar field and its
corresponding scalar metric perturbation, and gravitational waves that
are tensor metric fluctuations. The former experience gravitational
instability and lead to structure formation, while the latter can
influence the CMB anisotropies.  Defining slow-roll parameters (with
primes indicating derivatives with respect to the scalar field) as
$$
\epsilon = \frac{m_{{\rm Pl}}^2}{16\pi} \left( \frac{V'}{V} \right)^2 
\quad ,  \quad \eta = \frac{m_{{\rm Pl}}^2}{8\pi} \frac{V''}{V} \,,
\EQN{}
$$
which should satisfy $\epsilon,|\eta| \ll 1$, the spectra can be
computed using the slow-roll approximation as
$$
\Delta^2_{\cal R}(k)  \simeq  \left. \frac{8}{3 m_{{\rm Pl}}^4} \, 
\frac{V}{\epsilon} \right|_{k=aH} \quad , \quad
\Delta^2_{{\rm t}} (k) \simeq  \left. \frac{128}{3 m_{{\rm
Pl}}^4}  \, V \right|_{k=aH}\,.
\EQN{}
$$
In each case, the expressions on the right-hand side are to be
evaluated when the scale $k$ is equal to the Hubble radius during
inflation. The symbol `$\simeq$' here indicates use of the slow-roll
approximation, which is expected to be accurate to a few percent or
better.

From these expressions, we can compute the spectral
indices\cite{hubble:LL}:
$$
n_{{\rm s}} \simeq 1-6\epsilon + 2\eta \quad ; \quad n_{{\rm t}} \simeq
-2\epsilon \,. 
\EQN{}
$$
Another useful quantity is the ratio of the two spectra, defined by
$$
r \equiv \frac{\Delta^2_{{\rm t}} (k_*)}{\Delta^2_{\cal R}(k_*)} \,.
\EQN{}
$$
We have
$$
r \simeq 16 \epsilon \simeq - 8 n_{{\rm t}} \,,
\EQN{}
$$
which is known as the consistency equation.

One could consider corrections to the power-law approximation, which
we discuss later. However, for now we make the working assumption that
the spectra can be approximated by such power laws. The consistency
equation shows that $r$ and $n_{{\rm t}}$ are not independent
parameters, and so the simplest inflation models give initial
conditions described by three parameters, usually taken as
$\Delta^2_{{\cal R}}$, $n_{{\rm s}}$, and $r$, all to be evaluated at
some scale $k_*$, usually the `statistical center' of the range
explored by the data.  Alternatively, one could use the
parametrization $V$, $\epsilon$, and $\eta$, all evaluated at a point
on the putative inflationary potential.
 
After the perturbations are created in the early Universe, they
undergo a complex evolution up until the time they are observed in the
present Universe.  When the perturbations are small, this can be
accurately followed using a linear theory numerical code such as CAMB
or CLASS\cite{hubble:Boltz}. This works right up to the present for
the CMB, but for density perturbations on small scales non-linear
evolution is important and can be addressed by a variety of
semi-analytical and numerical techniques. However the analysis is
made, the outcome of the evolution is in principle determined by the
cosmological model and by the parameters describing the initial
perturbations, and hence can be used to determine them.

Of particular interest are CMB anisotropies. Both the total intensity
and two independent polarization modes are predicted to have
anisotropies. These can be described by the radiation angular power
spectra $C_\ell$ as defined in the CMB article in this volume, and
again provide a complete description if the density perturbations are
Gaussian.

\subsection{The standard cosmological model}
\IndexEntry{hubbleStandard}

\labelsubsection{params}

We now have most of the ingredients in place to describe the
cosmological model.  Beyond those of the previous subsections, we need
a measure of the ionization state of the Universe. The Universe is
known to be highly ionized at low redshifts (otherwise radiation from
distant quasars would be heavily absorbed in the ultra-violet), and
the ionized electrons can scatter microwave photons, altering the
pattern of observed anisotropies. The most convenient parameter to
describe this is the optical depth to scattering $\tau$ (\ie,~the
probability that a given photon scatters once); in the approximation
of instantaneous and complete reionization, this could equivalently be
described by the redshift of reionization $z_{{\rm ion}}$.

As described in \Sec{comb}, models based on these parameters are able
to give a good fit to the complete set of high-quality data available
at present, and indeed some simplification is possible. Observations
are consistent with spatial flatness, and the inflation models so far
described automatically generate negligible spatial curvature, so we
can set $k = 0$; the density parameters then must sum to unity, and so
one of them can be eliminated. The neutrino energy density is often
not taken as an independent parameter; provided that the neutrino
sector has the standard interactions, the neutrino energy density,
while relativistic, can be related to the photon density using thermal
physics arguments, and a minimal assumption takes the neutrino mass
sum to be that of the lowest mass solution to the neutrino oscillation
constraints, namely $0.06 \, {\rm eV}$. In addition, there is no
observational evidence for the existence of tensor perturbations
(though the upper limits are fairly weak), and so $r$ could be set to
zero.  This leaves seven parameters, which is the smallest set that
can usefully be compared to the present cosmological data. This
model is referred to by various names, including
\IndexEntry{hubbleLCDM}\IndexEntry{hubbleConcord}$\LAMBDA$CDM, the 
concordance cosmology, and the standard cosmological model.

Of these parameters, only $\OMEGA_{\gamma}$ is accurately measured
directly.  The radiation density is dominated by the energy in the
CMB, and the COBE satellite FIRAS experiment determined its
temperature to be $T = 2.7255 \pm 0.0006 \, {\rm
K}$\cite{hubble:fix},\footnote{$^\ddagger$}{Unless stated otherwise,
all quoted uncertainties in this article are $1\sigma$/68\% confidence
and all upper limits are 95\% confidence.  Cosmological parameters
sometimes have significantly non-Gaussian uncertainties. Throughout we
have rounded central values, and especially uncertainties, from
original sources, in cases where they appear to be given to excessive
precision.}  corresponding to $\OMEGA_{\gamma} = 2.47 \times 10^{-5}
h^{-2}$. It typically can be taken as fixed when fitting other data. Hence
the minimum number of cosmological parameters varied in fits to data
is six, though as described below there may additionally be many
`nuisance' parameters necessary to describe astrophysical processes
influencing the data.

In addition to this minimal set, there is a range of other parameters
that might prove important in future as the data-sets further improve,
but for which there is so far no direct evidence, allowing them to be
set to specific values for now.  We discuss various speculative
options in the next section. For completeness at this point, we
mention one other interesting quantity, the helium fraction, which is
a non-zero parameter that can affect the CMB anisotropies at a subtle
level.  It is usually fixed in microwave anisotropy studies, but the
data are approaching a level where allowing its variation may become
mandatory.

Most attention to date has been on parameter estimation, where a set
of parameters is chosen by hand and the aim is to constrain
them. Interest has been growing towards the higher-level inference
problem of model selection, which compares different choices of
parameter sets. Bayesian inference offers an attractive framework for
cosmological model selection, setting a tension between model
predictiveness and ability to fit the data\cite{hubble:hobson}.


\subsection{Derived parameters}

The parameter list of the previous subsection is sufficient to give a
complete description of cosmological models that agree with
observational data. However, it is not a unique parameterization, and
one could instead use parameters derived from that basic
set. Parameters that can be obtained from the set given above include
the age of the Universe, the present horizon distance, the present
neutrino background temperature, the epoch of matter--radiation
equality, the epochs of recombination and decoupling, the epoch of
transition to an accelerating Universe, the baryon-to-photon ratio,
and the baryon-to-dark-matter density ratio.  In addition, the
physical densities of the matter components, $\OMEGA_i h^2$, are often
more useful than the density parameters.  The density perturbation
amplitude can be specified in many different ways other than the
large-scale primordial amplitude, for instance, in terms of its effect
on the CMB, or by specifying a short-scale quantity, a common choice
being the present linear-theory mass dispersion on a scale of $8 \,
h^{-1} {\rm Mpc}$, known as $\sigma_8$.

Different types of observation are sensitive to different subsets of
the full cosmological parameter set, and some are more naturally
interpreted in terms of some of the derived parameters of this
subsection than on the original base parameter set. In particular,
most types of observation feature degeneracies whereby they are unable
to separate the effects of simultaneously varying specific
combinations of several of the base parameters.


\section{Extensions to the standard model}
\IndexEntry{hubbleExtensions}

At present, there is no positive evidence in favor of extensions of
the standard model.  These are becoming increasingly constrained by
the data, though there always remains the possibility of trace effects
at a level below present observational capability.

\subsection{More general perturbations}

The standard cosmology assumes adiabatic, Gaussian
perturbations. Adiabaticity means that all types of material in the
Universe share a common perturbation, so that if the space-time is
foliated by constant-density hypersurfaces, then all fluids and fields
are homogeneous on those slices, with the perturbations completely
described by the variation of the spatial curvature of the
slices. Gaussianity means that the initial perturbations obey Gaussian
statistics, with the amplitudes of waves of different wavenumbers
being randomly drawn from a Gaussian distribution of width given by
the power spectrum. Note that gravitational instability generates
non-Gaussianity; in this context, Gaussianity refers to a property of
the initial perturbations, before they evolve.

The simplest inflation models, based on one dynamical field, predict
adiabatic perturbations and a level of non-Gaussianity that is too
small to be detected by any experiment so far conceived. For present
data, the primordial spectra are usually assumed to be power laws.

\subsubsection{Non-power-law spectra}

For typical inflation models, it is an approximation to take the
spectra as power laws, albeit usually a good one. As data quality
improves, one might expect this approximation to come under pressure,
requiring a more accurate description of the initial spectra,
particularly for the density perturbations. In general, one can expand
$\ln \Delta_{\cal R}^2$ as
$$
\ln \Delta_{\cal R}^2(k) = \ln \Delta_{\cal R}^2(k_*) + (n_{{\rm s},*}-1) \ln 
\frac{k}{k_*} + \frac{1}{2} 
\left. \frac{dn_{{\rm s}}}{d\ln k} \right|_* \ln^2 \frac{k}{k_*} + \cdots \,,
\EQN{}
$$
where the coefficients are all evaluated at some scale $k_*$. The term
$dn_{{\rm s}}/d\ln k|_*$ is often called the running of the spectral
index\cite{hubble:KT}.  Once non-power-law spectra are allowed, it is
necessary to specify the scale $k_*$ at which the spectral index is
defined.

\subsubsection{Isocurvature perturbations}

An isocurvature perturbation is one that leaves the total density
unperturbed, while perturbing the relative amounts of different
materials. If the Universe contains $N$ fluids, there is one growing
adiabatic mode and $N-1$ growing isocurvature modes (for reviews
see \Ref{hubble:PDP} and \Ref{hubble:mw}). These can be excited, for
example, in inflationary models where there are two or more fields
that acquire dynamically-important perturbations. If one field decays
to form normal matter, while the second survives to become the dark
matter, this will generate a cold dark matter isocurvature
perturbation.

In general, there are also correlations between the different modes,
and so the full set of perturbations is described by a matrix giving
the spectra and their correlations. Constraining such a general
construct is challenging, though constraints on individual modes are
beginning to become meaningful, with no evidence that any other than
the adiabatic mode must be non-zero.

\subsubsection{Seeded perturbations}

An alternative to laying down perturbations at very early epochs is
that they are seeded throughout cosmic history, for instance by
topological defects such as cosmic strings. It has long been excluded
that these are the sole original of structure, but they could
contribute part of the perturbation signal, current limits being just
a few percent\cite{hubble:planckXXV}. In particular, cosmic defects
formed in a phase transition ending inflation is a plausible scenario
for such a contribution.

\subsubsection{Non-Gaussianity}

Multi-field inflation models can also generate primordial
non-Gaussianity (reviewed, \eg, in \Ref{hubble:PDP}). The extra fields
can either be in the same sector of the underlying theory as the
inflaton, or completely separate, an interesting example of the latter
being the curvaton model\cite{hubble:curv}. Current upper limits on
non-Gaussianity are becoming stringent, but there remains strong
motivation to push down those limits and perhaps reveal trace
non-Gaussianity in the data. If non-Gaussianity is observed, its
nature may favor an inflationary origin, or a different one such as
topological defects.

\subsection{Dark matter properties}
\IndexEntry{hubbleDMA}

Dark matter properties are discussed in the Dark Matter chapter in
this volume.  The simplest assumption concerning the dark matter is
that it has no significant interactions with other matter, and that
its particles have a negligible velocity as far as structure formation
is concerned. Such dark matter is described as `cold,' and candidates
include the lightest supersymmetric particle, the axion, and
primordial black holes. As far as astrophysicists are concerned, a
complete specification of the relevant cold dark matter properties is
given by the density parameter $\OMEGA_{{\rm c}}$, though those
seeking to detect it directly need also to know its interaction
properties.

Cold dark matter is the standard assumption and gives an excellent fit
to observations, except possibly on the shortest scales where there
remains some controversy concerning the structure of dwarf galaxies
and possible substructure in galaxy halos.  It has long been excluded
for all the dark matter to have a large velocity dispersion, so-called
`hot' dark matter, as it does not permit galaxies to form; for thermal
relics the mass must be above about 1\,keV to satisfy this constraint,
though relics produced non-thermally, such as the axion, need not obey
this limit. However, in future further parameters might need to be
introduced to describe dark matter properties relevant to
astrophysical observations. Suggestions that have been made include a
modest velocity dispersion (warm dark matter) and dark matter
self-interactions. There remains the possibility that the dark matter
is comprized of two separate components, \eg, a cold one and a hot
one, an example being if massive neutrinos have a non-negligible
effect.

\subsection{Relativistic species}\IndexEntry{hubbleRelativisticSpecies}

The number of relativistic species in the young Universe (omitting
photons) is denoted $N_{\rm eff}$. In the standard cosmological model
only the three neutrino species contribute, and its baseline value is
assumed fixed at 3.045 (the small shift from 3 is because of a slight
predicted deviation from a thermal
distribution\cite{hubble:sp16}). However other species could
contribute, for example an extra neutrino, possibly of sterile type,
or massless Goldstone bosons or other scalars. It is hence interesting
to study the effect of allowing this parameter to vary, and indeed
although 3.045 is consistent with the data, most analyses currently
suggest a somewhat higher value (\eg, \Ref{hubble:Neff}).

\subsection{Dark energy}\IndexEntry{hubbleDarkEnergy}

While the standard cosmological model given above features a
cosmological constant, in order to explain observations indicating
that the Universe is presently accelerating, further possibilities
exist under the general headings of `dark energy' and `modified
gravity'. These topics are described in detail in the Dark Energy
chapter in this volume. This article focuses on the case of the
cosmological constant, since this simple model is a good match to
existing data. We note that more general treatments of dark
energy/modified gravity will lead to weaker constraints on other
parameters.

\subsection{Complex ionization history}

The full ionization history of the Universe is given by the ionization
fraction as a function of redshift $z$. The simplest scenario takes
the ionization to have the small residual value left after
recombination up to some redshift $z_{{\rm ion}}$, at which point the
Universe instantaneously reionizes completely. Then there is a
one-to-one correspondence between $\tau$ and $z_{{\rm ion}}$ (that
relation, however, also depending on other cosmological
parameters). An accurate treatment of this process will track separate
histories for hydrogen and helium.  While currently rapid ionization
appears to be a good approximation, as data improve a more complex
ionization history may need to be considered.

\subsection{Varying `constants'}

Variation of the fundamental constants of Nature over cosmological
times is another possible enhancement of the standard cosmology. There
is a long history of study of variation of the gravitational constant
$G_{{\rm N}}$, and more recently attention has been drawn to the
possibility of small fractional variations in the fine-structure
constant. There is presently no observational evidence for the former,
which is tightly constrained by a variety of measurements. Evidence
for the latter has been claimed from studies of spectral line shifts
in quasar spectra at redshift $z \approx 2$\cite{hubble:Webb}, but
this is presently controversial and in need of further observational
study.  


\subsection{Cosmic topology}

The usual hypothesis is that the Universe has the simplest topology
consistent with its geometry, for example that a flat universe extends
forever.  Observations cannot tell us whether that is true, but they
can test the possibility of a non-trivial topology on scales up to
roughly the present Hubble scale. Extra parameters would be needed to
specify both the type and scale of the topology; for example, a
cuboidal topology would need specification of the three principal axis
lengths and orientation. At present, there is no evidence for non-trivial cosmic
topology\cite{hubble:planck2015XVIII}.

\section{Cosmological Probes}

\labelsection{obs}

The goal of the observational cosmologist is to utilize astronomical
information to derive cosmological parameters.  The transformation
from the observables to the parameters usually involves many
assumptions about the nature of the data, as well as of the dark
sector.  Below we outline the physical processes involved in each of
the major probes, and the main recent results. The first two
subsections concern probes of the homogeneous Universe, while the
remainder consider constraints from perturbations.

In addition to statistical uncertainties we note three sources of
systematic uncertainties that will apply to the cosmological
parameters of interest: (i) due to the assumptions on the cosmological
model and its priors (\ie,~the number of assumed cosmological
parameters and their allowed range); (ii) due to the uncertainty in
the astrophysics of the objects (\eg,~light-curve fitting for
supernovae or the mass--temperature relation of galaxy clusters); and
(iii) due to instrumental and observational limitations (\eg,~the
effect of `seeing' on weak gravitational lensing measurements, or beam
shape on CMB anisotropy measurements).

These systematics, the last two of which appear as `nuisance
parameters', pose a challenging problem to the statistical analysis.
We attempt a statistical fit to the whole Universe with 6 to 12 parameters, but we
might need to include hundreds of nuisance parameters, some of them
highly correlated with the cosmological parameters of interest (for
example time-dependent galaxy biasing could mimic the growth of mass
fluctuations).  Fortunately, there is some astrophysical prior
knowledge on these effects, and a small number of physically-motivated
free parameters would ideally be preferred in the cosmological
parameter analysis.


\subsection{Measures of the Hubble constant}

In 1929, Edwin Hubble discovered the law of expansion of the Universe
by measuring distances to nearby galaxies.  The slope of the relation
between the distance and recession velocity is defined to be the
present-epoch
Hubble constant, $H_0$.  Astronomers argued for decades about the
systematic uncertainties in various methods and derived values over
the wide range $40 \, {\rm km} \, {\rm s}^{-1} \, {\rm Mpc}^{-1}\simlt
H_0 \simlt 100 \, {\rm km} \, {\rm s}^{-1} \, {\rm Mpc}^{-1}$.

\IndexEntry{hubbleCepheid} 
One of the most reliable results on the Hubble constant came from the
Hubble Space Telescope (HST) Key Project\cite{hubble:freedman}.  This study
used the empirical period--luminosity relation for Cepheid variable
stars, and calibrated a number of secondary distance
indicators\IndexEntry{hubbleSupernovae}---Type Ia Supernovae (SNe Ia),
the Tully--Fisher relation, surface-brightness fluctuations, and Type
II Supernovae.  This approach was further extended, based on HST observations of 70 long-period Cepheids in the Large Magellanic Cloud, combined with  Milky Way parallaxes and masers in NGC4258, to yield  
$ H_0 = 74.0 \pm1.4 \;{\rm km} \, {\rm s}^{-1} \, {\rm Mpc}^{-1}$\cite{hubble:riess19}\ (the SH0ES project).
The major sources of uncertainty in this result are thought to be due to the heavy
element abundance of the Cepheids and the distance to the fiducial
nearby galaxy, the Large Magellanic Cloud, relative to which all
Cepheid distances are measured.

Three other methods have been used recently. One is a 
 calibration of the tip of the red-giant branch applied
to Type Ia supernovae, the Carnegie--Chicago Hubble Programme (CCHP) finding
$ H_0 = 69.8 \pm0.8 \; {\rm (stat.)} \; \pm 1.7 \; {\rm (sys.)} \;{\rm km} \, {\rm s}^{-1} \, {\rm Mpc}^{-1}$\cite{hubble:freedman2019}.
The second uses the method of time delay in six gravitationally-lensed quasars, with the result 
$ H_0 = 73.3^{+1.7}_{-1.8} \;{\rm km} \, {\rm s}^{-1} \, {\rm Mpc}^{-1}$\cite{hubble:Holicow}\ (H0LiCOW).
A third method that came to fruition recently is based on gravitational waves; the `bright standard siren' applied to  the binary neutron star GW170817
and  the `dark standard siren' implemented on the binary black hole GW170814 yield
$ H_0 = 70^{+12}_{-8} \;{\rm km} \, {\rm s}^{-1} \, {\rm Mpc}^{-1}$\cite{hubble:bright_siren} 
and 
$ H_0 = 75^{+40}_{-32} \;{\rm km} \, {\rm s}^{-1} \, {\rm Mpc}^{-1}$\cite{hubble:dark_siren} respectively.
With many more gravitational-wave events the future uncertainties on $H_0$ from standard sirens will get smaller.

The determination of $H_0$ by the {\it Planck} Collaboration\cite{hubble:planck2018VI} gives a lower value, $H_0 =
67.4 \pm 0.5 \;{\rm km} \, {\rm s}^{-1} \, {\rm Mpc}^{-1}$.   As
discussed in their paper, there is strong degeneracy of $H_0$ with
other parameters, \eg, $\OMEGA_{\rm m}$ and the neutrino mass.  
It is worth noting that using the `inverse distance ladder' method gives a result $H_0 = 67.8 \pm 1.3  \;{\rm km} \, {\rm s}^{-1} \, {\rm Mpc}^{-1}$\cite{hubble:inverse_ladder} , close to the {\it Planck} result.
The inverse distance ladder relies on absolute-distance measurements from baryon acoustic oscillations (BAOs) to
calibrate the intrinsic magnitude of the SNe Ia (rather than by nearby Cepheids and parallax).
This measurement  was derived from 207  spectroscopically-confirmed Type Ia supernovae
from the Dark Energy Survey (DES), an additional 122 low-redshift  SNe Ia, and measurements of BAOs. 
A combination of DES Y1 clustering and weak lensing with  BAO and BBN (assuming $\LAMBDA$CDM) gives 
$ H_0 = 67.4^{+1.1}_{-1.2} \;{\rm km} \, {\rm s}^{-1} \, {\rm Mpc}^{-1}$\cite{hubble:DESY1_BAO_BBN} .

The tension between the $H_0$ values from {\it Planck} and the traditional cosmic
distance ladder methods is of great interest and under investigation.
For example, the SH0ES and H0LiCOW+SH0ES results deviate from {\it Planck} by $4.4\sigma$ and $5.3\sigma$ respectively,
while the TRGB and standard-siren results lie between the {\it Planck} and cosmic ladder $H_0$ values. 
There is possibly a trend for higher $H_0$ derived from the nearby Universe and a lower $H_0$ from the early Universe, which has led some researchers to propose a time-variation of the dark energy component or other exotic scenarios. Ongoing studies are addressing the question of whether the Hubble tension is due to systematics in at least one of the probes, or a signature of new physics. 

\Figure{H0} shows a selection of recent $H_0$ values, adapted from \Ref{verde} which provides a very useful summary of the current status of the Hubble constant tension.

\topfigure{H0}
\RPPfigurescaled{H0_plot_v2.eps}{center}{3in}%
{A selection of recent $H_0$ measurements from the various projects as described in the text, divided into early and late Universe probes. The standard-siren determinations are omitted as they are too wide for the plot. Figure courtesy of Vivien Bonvin and Martin Millon, adapted from \Ref{verde}.}
~\\ %To separate figure and caption better
\IndexEntry{hubbleColorFigOne}
\endfigure

%------------------------------------------------------------------------------------------------

\subsection{Supernovae as cosmological probes}

Empirically, the peak luminosity of SNe Ia can be used as an efficient
distance indicator (\eg,~\Ref{hubble:leibundgut}), thus allowing
cosmology to be constrained via the distance--redshift relation.  The
favorite theoretical explanation for SNe Ia is the thermonuclear
disruption of carbon--oxygen white dwarfs.  Although not perfect
`standard candles', it has been demonstrated that by correcting for a
relation between the light-curve shape, color, and luminosity at
maximum brightness, the dispersion of the measured luminosities can be
greatly reduced.  There are several possible systematic effects that
may affect the accuracy of the use of SNe Ia as distance indicators,
\eg, evolution with redshift and interstellar extinction in
the host galaxy and in the Milky Way.

Two major studies, the Supernova Cosmology Project and the High-$z$
Supernova Search Team, found evidence for an accelerating
Universe\cite{hubble:snfirst}, interpreted as due to a cosmological
constant or a dark energy component.  When combined with the CMB data
(which indicate near flatness, \ie, $\OMEGA_{{\rm m}} +
\OMEGA_{\LAMBDA} \simeq 1$), the best-fit values were $\OMEGA_{{\rm
m}} \approx 0.3 $ and $\OMEGA_{\LAMBDA} \approx 0.7 $.  Most results
in the literature are consistent with the $w=-1$ cosmological constant
case.  One study\cite{hubble:betoule14}deduced, from a sample of
740 spectroscopically-confirmed SNe Ia, that $\OMEGA_{\rm m} =
0.295 \pm 0.034$ (stat+sym) for an assumed flat $\LAMBDA$CDM model.
An analysis of a  sample of spectroscopically-confirmed  207 DES SNe Ia combined with 122 low-redshift  SNe\cite{hubble:DES_SNeIa}
yielded $\OMEGA_{\rm m} = 0.331 \pm 0.038$  for an assumed flat $\LAMBDA$CDM model.
In combination with the CMB, for a flat $w$CDM these data give $w=-0.978 \pm 0.059$ and $\OMEGA_{\rm m} = 0.321 \pm 0.018$, consistent with results from the JLA and Pantheon SNe Ia samples.
Future experiments will refine constraints on the cosmic equation of state $w(z)$.

\subsection{Cosmic microwave background}
\IndexEntry{hubbleCMB}

The physics of the CMB is described in detail in the CMB chapter in
this volume. Before recombination, the baryons and photons are tightly
coupled, and the perturbations oscillate in the potential wells
generated primarily by the dark matter perturbations. After
decoupling, the baryons are free to collapse into those potential
wells.  The CMB carries a record of conditions at the time of last
scattering, often called primary anisotropies. In addition, it is
affected by various processes as it propagates towards us, including
the effect of a time-varying gravitational potential (the integrated
Sachs--Wolfe effect), gravitational lensing, and scattering from
ionized gas at low redshift.

\IndexEntry{hubbleCBranis}
\IndexEntry{hubbleSW}
The primary anisotropies, the integrated Sachs--Wolfe effect, and the
scattering from a homogeneous distribution of ionized gas, can all be
calculated using linear perturbation theory. Available codes include
CAMB and CLASS\cite{hubble:Boltz}, the former widely used embedded
within the analysis package CosmoMC\cite{hubble:LewBrid} 
and in higher-level analysis packages such as
CosmoSIS\cite{hubble:cosmosis} and CosmoLike\cite{hubble:cosmolike}.
Gravitational lensing is also calculated in these codes. Secondary
effects, such as inhomogeneities in the reionization process, and
scattering from gravitationally-collapsed gas
\IndexEntry{hubbleSZeldovich}(the Sunyaev--Zeldovich or SZ effect), 
require more complicated, and more uncertain, calculations.

The upshot is that the detailed pattern of anisotropies depends on all
of the cosmological parameters. In a typical cosmology, the anisotropy
power spectrum [usually plotted as $\ell(\ell+1)C_\ell$] features a
flat plateau at large angular scales (small $\ell$), followed by a
series of oscillatory features at higher angular scales, the first and
most prominent being at around one degree ($\ell \simeq 200$). These
features, known as acoustic peaks, represent the oscillations of the
photon--baryon fluid around the time of decoupling. Some features can
be closely related to specific parameters---for instance, the location
in multipole space of the set of peaks probes the spatial geometry,
while the relative heights of the peaks probe the baryon density---but
many other parameters combine to determine the overall shape.

\IndexEntry{hubblePlanck}\IndexEntry{hubbleWMAP}
The 2018 data release from the {\it Planck}
satellite\cite{hubble:planck2018I} gives the most powerful results to date
on the spectrum of CMB temperature anisotropies, with a precision
determination of the temperature power spectrum to beyond $\ell =
2000$. The Atacama Cosmology Telescope (ACT) and South Pole Telescope
(SPT) experiments extend these results to higher angular resolution,
though without full-sky coverage. {\it Planck} and the polarisation-sensitive versions of ACT and SPT
give the
state of the art in measuring the spectrum of $E$-polarization
anisotropies and the correlation spectrum between temperature and
polarization. These are consistent with models based on the
parameters we have described, and provide accurate determinations of
many of those parameters\cite{hubble:planck2018VI}. Primordial
$B$-mode polarization has not been detected (although the
gravitational lensing effect on $B$ modes has been measured).

The data provide an exquisite measurement of the location of the set
of acoustic peaks, determining the angular-diameter distance of the
last-scattering surface. In combination with other data this strongly
constrains the spatial geometry, in a manner consistent with spatial
flatness and excluding significantly-curved Universes.  CMB data give
a precision measurement of the age of the Universe. The CMB also gives
a baryon density consistent with, and at higher precision than, that
coming from BBN. It affirms the need for both dark matter and dark
energy.  It shows no evidence for dynamics of the dark energy, being
consistent with a pure cosmological constant ($w = -1$).  The density
perturbations are consistent with a power-law primordial spectrum, and
there is no indication yet of tensor perturbations.
\IndexEntry{hubbleReIon} 
The current best-fit for the reionization optical depth from CMB data,
$\tau = 0.054$, is in line with models of how early structure
formation induces reionization.

{\it Planck} has also made the first all-sky map of the CMB lensing
field, which probes the entire matter distribution in the Universe and
adds some additional constraining power to the CMB-only data-sets. These measurements are compatible with the
expected effect in the standard cosmology.

\subsection{Galaxy clustering}
\IndexEntry{hubbleGalaxyClustering}
\labelsubsection{bias}

The power spectrum of density perturbations is affected by the nature of
the dark matter.  Within the $\LAMBDA$CDM model, the power spectrum
shape depends primarily on the primordial power spectrum and on the
combination $\OMEGA_{{\rm m}} h$, which determines the horizon scale
at matter--radiation equality, with a subdominant dependence on the
baryon density.  The matter distribution is most easily probed by
observing the galaxy distribution, but this must be done with care
since the galaxies do not perfectly trace the dark matter
distribution.  Rather, they are a `biased' tracer of the dark
matter\cite{hubble:Kaiser84}.  The need to allow for such bias is
emphasized by the observation that different types of galaxies show
bias with respect to each other.  In particular, scale-dependent and
stochastic biasing may introduce a systematic effect on the
determination of cosmological parameters from redshift
surveys\cite{hubble:DL99}.  Prior knowledge from simulations of galaxy
formation or from gravitational lensing data could help to quantify
biasing.  Furthermore, the observed 3D galaxy distribution is in
redshift space, \ie, the observed redshift is the sum of the Hubble
expansion and the line-of-sight peculiar velocity, leading to linear
and non-linear dynamical effects that also depend on the cosmological
parameters.  On the largest length scales, the galaxies are expected
to trace the location of the dark matter, except for a constant
multiplier $b$ to the power spectrum, known as the linear bias
parameter.  On scales smaller than 20 Mpc or so, the
clustering pattern is `squashed' in the radial direction due to
coherent infall, which depends approximately on the parameter
$\beta \equiv \OMEGA_{{\rm m}}^{0.6}/b$ (on these shorter scales, more
complicated forms of biasing are not excluded by the data).  On scales
of a few Mpc, there is an effect of elongation along the line
of sight (colloquially known as the `finger of God' effect) that
depends on the galaxy velocity dispersion.

\subsubsection{Baryon acoustic oscillations} 
\IndexEntry{hubbleGalPwrSpec}

The power spectra of the 2-degree Field (2dF) Galaxy Redshift Survey
and the Sloan Digital Sky Survey (SDSS) are well fit by a $\LAMBDA$CDM
model and both surveys showed first evidence for baryon acoustic
oscillations (BAOs)\cite{hubble:eisenstein05}\cite{hubble:cole05}.
The Baryon Oscillation Spectroscopic Survey (BOSS) of luminous red
galaxies (LRGs) in the SDSS (DR 12) found, using a sample of 1.2 million galaxies,  consistency with  $w=-1.01 \pm 0.06$\cite{hubble:boss17} when combined with {\it Planck} 2015.  Similar results for $w$
were obtained by the WiggleZ survey\cite{hubble:parkinson13}.


\subsubsection{Redshift distortion}

There is renewed interest in the `redshift distortion' effect.  This
distortion depends on cosmological parameters\cite{hubble:kaiser} via
the perturbation growth rate in linear theory $f(z) = d \ln \delta
/d \ln a \approx \OMEGA^\gamma(z)$, where $\gamma
\simeq 0.55$ for the $\LAMBDA$CDM model and may be different for 
modified gravity models.  By measuring $f(z)$ it is feasible to
constrain $\gamma$ and rule out certain modified gravity
models\cite{hubble:guzzo}\cite{hubble:nusser11}. We note the
degeneracy of the redshift-distortion pattern and the geometric
distortion (the so-called Alcock--Paczynski
effect\cite{hubble:ap1979})$\!\!$, %Fix by hand to remove space
                                %before full stop generated by \cite 
\eg, as illustrated by the WiggleZ
survey\cite{hubble:blake12}
and the BOSS Survey\cite{hubble:BOSS16}.


\IndexEntry{hubbleSDSS}

\subsubsection{Limits on neutrino mass from galaxy surveys and other
probes}
\labelsubsection{neut2dF}

\IndexEntry{hubbleNuMass} 

Large-scale structure data place constraints on $\OMEGA_{\nu}$ due to
the neutrino free-streaming effect\cite{hubble:lp06}.  Presently there
is no clear detection, and upper limits on neutrino mass are commonly
estimated by comparing the observed galaxy power spectrum with a
four-component model of baryons, cold dark matter, a cosmological
constant, and massive neutrinos.  Such analyses also assume that the
primordial power spectrum is adiabatic, scale-invariant, and Gaussian.
Potential systematic effects include biasing of the galaxy
distribution and non-linearities of the power spectrum.  An upper
limit can also be derived from CMB anisotropies alone, while
combination with additional cosmological data-sets can improve the
results.

The most recent results on neutrino mass upper limits and other
neutrino properties are summarised in the Neutrinos in Cosmology
chapter in this volume.  While the latest cosmological data do not yet
constrain the sum of neutrino masses to below 0.2 eV, since the lower
limit on this sum from oscillation experiments is 0.06 eV it is
expected that future cosmological surveys will soon detect effects
from the neutrino mass.  Also, current cosmological datasets are in
good agreement with the standard value for the effective number of
neutrino species $N_{\rm eff} = 3.045$.

\subsection{Clustering in the inter-galactic medium}

It is commonly assumed, based on hydrodynamic simulations, that the
neutral hydrogen in the inter-galactic medium (IGM) can be related to
the underlying mass distribution.  It is then possible to estimate the
matter power spectrum on scales of a few megaparsecs from the
absorption observed in quasar spectra, the so-called Lyman-$\alpha$
forest.  The usual procedure is to measure the power spectrum of the
transmitted flux, and then to infer the mass power spectrum.
Photo-ionization heating by the ultraviolet background radiation and
adiabatic cooling by the expansion of the Universe combine to give a
simple power-law relation between the gas temperature and the baryon
density.  It also follows that there is a power-law relation between
the optical depth $\tau$ and $\rho_{{\rm b}}$.  Therefore, the
observed flux $F = \exp(-\tau)$ is strongly correlated with
$\rho_{{\rm b}}$, which itself traces the mass density.  The matter
and flux power spectra can be related by a biasing function that is
calibrated from simulations.  

A  study of 266,590 quasars in the range $1.77 < z < 3$ 
from SDSS was used to measure the BAO scale from the 3D correlation of Lyman-$\alpha$ and quasars\cite{hubble:lya1}.
Combined with the Lyman-$\alpha$  auto-correlation measurement presented in a companion paper\cite{hubble:lya2} 
 the BAO measurements at $z=2.34$ are within 1.7$\sigma$  of the {\it Planck} 2018 $\LAMBDA$CDM model. The Lyman-$\alpha$
flux power spectrum has also been used to constrain the nature of dark
matter, for example limiting the amount of warm dark
matter\cite{hubble:viel13}.


\topfigure{KiDS}
\RPPfigure{KiDS-S8Om.eps}{center}
{Marginalised posterior contours (inner 68\% confidence level, outer 95\% confidence level) in the  $\OMEGA_{{\rm m}}$--$S_8$ 
 plane. Shown are 
 the optical-only KiDS-450 analysis (green; \Ref{hubble:KiDS18}),  the fiducial KiDS+VISTA-450 setup (blue; \Ref{hubble:KiDS18}), DES Year 1 using cosmic shear only (purple; \Ref{hubble:Troxel18}),
 %Troxel et al. 2018b, 
 HSC-DR1 cosmic shear (orange;  \Ref{hubble:Higake18})
 %Hikage et al. 2018), 
 and the {\it Planck} Legacy analysis
 (red; {\it Planck} Collaboration\cite{hubble:planck2018VI}  using TT+TE+EE+lowE). Figure from \Ref{hubble:KiDS18}. }
~\\ %To separate figure and caption better
\IndexEntry{hubbleColorFigTwo}
\endfigure

\subsection{Weak gravitational lensing}
\IndexEntry{hubbleGravLens}

Images of background galaxies are distorted by the gravitational
effect of mass variations along the line of sight.  Deep gravitational
potential wells, such as galaxy clusters, generate `strong lensing'
leading to arcs, arclets, and multiple images, while more moderate
perturbations give rise to `weak lensing'.  Weak lensing is now widely
used to measure the mass power spectrum in selected regions of the sky
(see \Ref{hubble:lensing} for reviews).  Since the signal is weak, the
image of deformed galaxy shapes (the `shear map') must be analyzed
statistically to measure the power spectrum, higher moments, and
cosmological parameters.  There are various systematic effects in the
interpretation of weak lensing, \eg, due to atmospheric distortions
during observations, the redshift distribution of the background
galaxies (usually depending on the accuracy of photometric redshifts), the intrinsic correlation of galaxy shapes, and non-linear
modeling uncertainties. 

As one example, the  `Kilo-Degree Survey' (KiDS), combined with the  VISTA VIKING survey, 
used weak-lensing measurements over 450 deg$^2$ to constrain the clumpiness parameter
$S_8 \equiv \sigma_8 (\OMEGA_{{\rm m}}/0.3)^{0.5} = 0.737^{+0.040}_{-0.036}$\cite{hubble:KiDS18} .
This is lower by $2.3\sigma$ than $S_8$ derived from {\it Planck}. 
\Figure{KiDS} (which is Figure 4 from \Ref{hubble:KiDS18}) 
shows the  $\OMEGA_{{\rm m}}$--$S_8$  constraints derived from weak lensing of KiDS, DES, and HPC versus the CMB constraint from {\it Planck}.
Variations in $S_8$ among the weak-lensing surveys are mainly due to difference in the procedures for photometric redshift determinations. 
Results from weak lensing from DES, combined with other probes, are shown in the next section.


\subsection{Other probes}

Other probes that have been used to constrain cosmological parameters,
but that are not presently competitive in terms of accuracy, are the
integrated Sachs--Wolfe
effect\cite{hubble:isw1}\cite{hubble:planckXXI}, the number density or
composition of galaxy clusters\cite{hubble:planckXXIV}, and galaxy
peculiar velocities, which probe the mass fluctuations in the local
Universe\cite{hubble:dekel}.

\section{Bringing probes together}

\labelsection{comb}

% Maybe also say something about ?precision? vs ?accuracy? 

Although it contains two ingredients---dark matter and dark
energy---which have not yet been verified by laboratory experiments,
the $\LAMBDA$CDM model is almost universally accepted by cosmologists
as the best description of the present data. The approximate values of
some of the key parameters are $\OMEGA_{{\rm b}} \approx 0.05$,
$\OMEGA_{{\rm c}} \approx 0.25$, $\OMEGA_{\LAMBDA} \approx 0.70$, and
a Hubble constant $h \approx 0.70$. The spatial geometry is very close
to flat (and usually assumed to be precisely flat), and the initial
perturbations Gaussian, adiabatic, and nearly scale-invariant.
  
The most powerful data source is the CMB, which on its own supports
all these main tenets. Values for some parameters, as given
in \Ref{hubble:planck2018VI}, are reproduced
in \Table{constraints}. These particular results presume a flat
Universe.  The constraints are somewhat strengthened by adding
additional data-sets,  BAO being shown in the
Table as an example, though most of the constraining power resides in the CMB
data. Similar constraints at lower precision were previously obtained by the {\it WMAP}
collaboration.

\toptable{constraints}
\Caption
Parameter constraints reproduced from \Ref{hubble:planck2018VI}
(Table 2, column 5), with some additional rounding.  Both columns assume the
$\LAMBDA$CDM cosmology with a power-law initial spectrum, no tensors,
spatial flatness, a cosmological constant as dark energy, and the sum
of neutrino masses fixed to 0.06 eV. Above the line are the six
parameter combinations actually fit to the data ($\theta_{\rm MC}$ is
a measure of the sound horizon at last scattering); those below the
line are derived from these.  The first column uses {\it Planck}
primary CMB data plus the {\it
Planck} measurement of CMB lensing. This column gives our present
recommended values. The second column adds in data from a compilation of BAO measurements described in  \Ref{hubble:planck2018VI}.  The
perturbation amplitude $\Delta^2_{\cal R}$ (denoted $A_{\rm s}$ in the
original paper) is specified at the scale $0.05 \, {\rm Mpc}^{-1}$.
Uncertainties are shown at 68\% confidence.
\endCaption
\centerline{\vbox{
\tabskip=0pt\baselineskip 22pt
\halign  {\strut#&\tabskip=1em plus 1em minus 0.5em% 
               %1st column is strut
             \lefttab{#}&           % 2nd column is text FIRST
             \centertab{#}&           % 2nd column is text FIRST
             \centertab{#}&           % 3rd column is text FIRST
             \centertab{#}\tabskip=0pt\cr % 7th text FOURTH
\tableheaddoublerule%_______________________________________
%___________________________________________________________
&&   {\it Planck} TT,TE,EE+lowE+lensing  & +BAO \cr
\tableheadsinglerule%_______________________________________
&$\OMEGA_{{\rm b}} h^2$ & $0.02237 \pm 0.00015$ & $0.02242 \pm 0.00014$ \cr
&$\OMEGA_{{\rm c}} h^2$ & $0.1200 \pm 0.0012$ & $0.1193 \pm 0.0009$ \cr
&$100 \,\theta_{\rm MC}$ & $1.0409 \pm 0.0003$ & $1.0410 \pm 0.0003$ \cr
&$n_{{\rm s}}$ & $0.965 \pm 0.004$ & $0.966 \pm 0.004$ \cr
&$\tau$ & $0.054 \pm 0.007$ & $0.056 \pm 0.007$ \cr
&$\ln(10^{10}\Delta^2_{\cal R})$ & $3.044 \pm 0.014$ & $3.047 \pm 0.014$ \cr
\tableheadsinglerule
&$h$ & $0.674 \pm 0.005$ & $0.677\pm 0.004$ \cr
&$\sigma_8$ & $0.811 \pm 0.006$ & $0.810 \pm 0.006$ \cr
&$\OMEGA_{{\rm m}}$ & $0.315 \pm 0.007$ & $0.311 \pm 0.006$ \cr
&$\OMEGA_\LAMBDA$ & $0.685 \pm 0.007$ & $0.689 \pm 0.006$  \cr
\tablefootdoublerule%_______________________________________
%___________________________________________________________
}}}
\endtable

If the assumption of spatial flatness is lifted, it turns out that the
primary CMB on its own constrains the spatial curvature fairly weakly, due to a
parameter degeneracy in the angular-diameter distance. However,
inclusion of other data readily removes this degeneracy. Simply adding the {\it Planck} lensing measurement, and with the assumption that the dark energy is a
cosmological constant, yields a 68\% confidence constraint on
\IndexEntry{hubbleTotDen} $\OMEGA_{{\rm tot}} \equiv 
\sum \OMEGA_i + \OMEGA_\LAMBDA  = 1.011 \pm
0.006$ and further adding BAO makes it $0.9993 \pm 0.0019$\cite{hubble:planck2018VI}.  Results of this type are
normally taken as justifying the restriction to flat cosmologies.

\IndexEntry{hubbleAgeUniverse}
One derived parameter that is very robust is the age of the Universe,
since there is a useful coincidence that for a flat Universe the
position of the first peak is strongly correlated with the age.  The
CMB data give $13.797 \pm 0.023$ Gyr (assuming flatness).  This is in
good agreement with the ages of the oldest globular clusters and with
radioactive dating.
 
The baryon density $\OMEGA_{\rm b}$ is now measured with high accuracy
from CMB data alone, and is consistent with and much more precise than
the determination from BBN.  The value quoted in the Big-Bang
Nucleosynthesis chapter in this volume is $0.021 \le \OMEGA_{{\rm b}}
h^2 \le 0.024$ (95\% confidence).

While $\OMEGA_\LAMBDA$ is measured to be non-zero with very high
confidence, there is no evidence of evolution of the dark energy
density.  As described in the Dark Energy chapter in this volume, from
a combination of CMB, weak gravitational lensing, SN, and BAO measurements, assuming a flat
universe, \Ref{hubble:planck2018VI} found $w=-1.028 \pm 0.031$, consistent with the
cosmological constant case $w = -1$.  Allowing more complicated forms
of dark energy weakens the limits.
  
The data provide strong support for the main predictions of the
simplest inflation models: spatial flatness and adiabatic, Gaussian,
nearly scale-invariant density perturbations. But it is disappointing
that there is no sign of primordial gravitational waves, with a 95\% confidence upper
limit from combining {\it Planck} with BICEP2/Keck Array BK15 data of $r<0.06$ at the scale $0.002 \, {\rm Mpc}^{-1}$ \cite{hubble:planck2018X}\ (weakening somewhat if running is
allowed). The spectral index is clearly required to be less than one
by current data, though the strength of that conclusion can weaken if
additional parameters are included in the model fits.

Tests have been made for various types of non-Gaussianity, a
particular example being a parameter $f_{{\rm NL}}$ that measures a
quadratic contribution to the perturbations. Various non-Gaussian
shapes are possible (see \Ref{hubble:planck2018IX} for details), and
current constraints on the popular `local', `equilateral', and
`orthogonal' types (combining temperature and polarization data) are $
f^{{\rm local}}_{{\rm NL}} = -1 \pm 5$, $f^{{\rm equil}}_{{\rm NL}} =
-26 \pm 47$, and $f^{{\rm ortho}}_{{\rm NL}} = -38 \pm 24$ respectively
(these look weak, but prominent non-Gaussianity requires the product
$f_{{\rm NL}}\Delta_{\cal R}$ to be large, and $\Delta_{\cal R}$ is of
order $10^{-5}$). Clearly none of these give any indication of
primordial non-gaussianity.

While the above results come from the CMB alone, other probes are
becoming competitive (especially when considering more complex
cosmological models), and so combination of data from different sources is of growing
importance.  We note that it has become fashionable to combine probes
at the level of power-spectrum data vectors, taking into account
nuisance parameters in each type of measurement.  Recent examples include
KiDS+GAMA\cite{hubble:KiDS} and Dark Energy Survey (DES) Year
1\cite{hubble:DESY1}. For example, the DES analysis includes galaxy
position--position clustering, galaxy--galaxy lensing, and weak
lensing shear.  Discussions on `tension' in resulting cosmological
parameters depend on the statistical approaches used. Commonly the
cosmology community works within the Bayesian framework, and assesses
agreement amongst data sets with respect to a model via Bayesian
Evidence, essentially the denominator in Bayes's theorem.  As an
example of results, combining DES Y1 with {\it Planck}, BAO measurements from SDSS, 6dF, and BOSS, and type
Ia supernovae from the Joint Lightcurve Analysis (JLA) dataset has
shown the datasets to be mutually compatible and yields very tight
constraints on cosmological parameters: $S_8 \equiv \sigma_8
(\OMEGA_{{\rm m}}/0.3)^{0.5} = 0.799^{+0.014}_{-0.009}$, and
$\OMEGA_{{\rm m}} = 0.301^{+0.006}_{-0.008}$ in $\LAMBDA$CDM, and
$w=-1.00^{+0.04}_{-0.05}$ in $w$CDM\cite{hubble:DESY1}. The combined
measurement of the Hubble constant within $\LAMBDA$CDM gives
$H_0= 68.2\pm0.6 \;{\rm km} \, {\rm s}^{-1} \, {\rm Mpc}^{-1}$, still leaving some level of tension with the local
measurements described earlier. Future analyses and the next
generation of surveys will test for deviations from $\LAMBDA$CDM, for
example epoch-dependent $w(z)$ and modifications to General
Relativity.


\section{Outlook for the future}

The concordance model is now well established, and there seems little
room left for any dramatic revision of this paradigm. A measure of the
strength of that statement is how difficult it has proven to formulate
convincing alternatives.

Should there indeed be no major revision of the current paradigm, we
can expect future developments to take one of two directions. Either
the existing parameter set will continue to prove sufficient to
explain the data, with the parameters subject to ever-tightening
constraints, or it will become necessary to deploy new parameters. The
latter outcome would be very much the more interesting, offering a
route towards understanding new physical processes relevant to the
cosmological evolution. There are many possibilities on offer for
striking discoveries, for example:
\itemize
\itm the cosmological effects of a neutrino mass may be unambiguously
detected, shedding light on fundamental neutrino properties;
\itm detection of primordial non-Gaussianities would indicate that
non-linear processes influence the perturbation generation mechanism;
\itm detection of variation in the dark-energy density (\ie,~$w \neq
-1$) would provide much-needed experimental input into its nature.
\enditemize
\noindent
These provide more than enough motivation for continued efforts to
test the cosmological model and improve its accuracy.
Over the coming years, there are a wide range of new observations
that  will bring further precision to cosmological studies. Indeed,
there are far too many for us to be able to mention them all here, and
so we will just highlight a few areas.

The CMB observations will improve in several directions.  A current
frontier is the study of polarization, for which power spectrum
measurements have now been made by several experiments. Detection of
primordial $B$-mode anisotropies is the next major goal and a variety
of projects are targeting this, though theory gives little guidance as
to the likely signal level. 
Future CMB projects that are approved include {\it LiteBIRD} and the Simons Observatory.

An impressive array of cosmology surveys are already operational, under
construction, or proposed, including the ground-based Hyper Suprime Camera (HSC) and Large Synoptic Survey
Telescope (LSST) imaging surveys, spectroscopic surveys such as the
Dark Energy Spectroscopic Instrument (DESI), and space missions {\it Euclid}
and the Wide-Field Infrared Survey (WFIRST).

An exciting area for the future is radio surveys of the redshifted
21-cm line of hydrogen. Because of the intrinsic narrowness of this
line, by tuning the bandpass the emission from narrow redshift slices
of the Universe will be measured to extremely high redshift, probing
the details of the reionization process at redshifts up to perhaps 20,
as well as measuring large-scale features such as the BAOs.  LOFAR and CHIME are
the first instruments able to do this and have begun operations. In
the longer term, the Square Kilometre Array (SKA) will take these
studies to a precision level.

The development of the first precision cosmological model is a major
achievement. However, it is important not to lose sight of the
motivation for developing such a model, which is to understand the
underlying physical processes at work governing the Universe's
evolution. From that perspective, progress has been much less dramatic. For
instance, there are many proposals for the nature of the dark matter,
but no consensus as to which is correct. The nature of the dark energy
remains a mystery. Even the baryon density, now measured to an
accuracy of a percent, lacks an underlying theory able to predict it
within orders of magnitude. Precision cosmology may have arrived, but
at present many key questions remain to motivate and challenge the
cosmology community.


\smallskip
\noindent{\bf References:}

\smallskip
\parindent=20pt
\ListReferences
\vfill\eject
        

\endRPPonly


==> hubble-def.tex <==
%DEFINITIONS FOR HUBBLE
\def\bolditalicx{\hbox{\bf\tenmib{x}}}
\def\bolditalick{\hbox{\bf\tenmib{k}}}
\beginRPPonly
\def\shortstrut{\vrule height 10pt depth 4pt width 0pt}
\endRPPonly
\beginDBonly
\def\shortstrut{\vrule height 9pt depth 3pt width 0pt}
\endDBonly

